Avoiding algebraic integers of bounded house in orbits of rational functions over cyclotomic closures

Let $k$ be a number field with cyclotomic closure $k^{\mathrm{cyc}}$, and let $h \in k^{\mathrm{cyc}}(x)$. For $A \ge 1$ a real number, we show that \[ \{ \alpha \in k^{\mathrm{cyc}} : h(\alpha) \in \overline{\mathbb Z} \text{ has house at most } A \} \] is finite for many $h$. We also show that for many such $h$ the same result holds if $h(\alpha)$ is replaced by orbits $h(h(\cdots h(\alpha)))$. This generalizes a result proved by Ostafe that concerns avoiding roots of unity, which is the case $A=1$.

==> flowchart.tex <==
\appendix
\section{Graph of dependencies}
\label{sec:flowchart}
The following graph shows the dependencies
among the various numbered results in the paper,
and implicitly where certain hypothesis are used.

\begin{center}
% Define block styles
\tikzstyle{every node}=[font=\small]
\tikzstyle{arrow} = [draw, -{>[scale=2]},
	shorten >= 2pt, shorten <= 2pt]
\tikzstyle{tool} = [draw, rounded corners,
	fill=red!10, node distance=4.5cm,
	minimum height=2em]
\tikzstyle{thm} = [rectangle, draw, fill=blue!10,
	node distance=4.5cm, text width=6em,
	minimum height=5em]
\begin{tikzpicture}[node distance = 1.5cm, auto]
	% Place nodes
	\node [thm, text width = 8em] (n25) {\textbf{2.5.} $h$ is $P_A$-avoiding unless $A$-short witness};
	\node [thm, left of = n25] (n14) {\textbf{1.4.} More than $2$ poles implies $P_A$-avoiding};
	\node [thm, right of = n25] (n27) {\textbf{2.7.} If $\deg h \gg 1$ then assume $\deg S \le 2$};

	\node [tool, above of = n25, anchor = east, text width = 4em, shift={(-0.7,0)}] (n21) {\textbf{2.1-2.4.} Loxton};
	\node [tool, above of = n25, anchor = west, text width = 4em, shift={(0.7,0)}] (n31) {\textbf{3.1-3.2.} On $\BG^d$};
	\node [tool, text width = 5em, above of = n27] (n33) {\textbf{3.3.} Terms in $p = h \circ q$};

	\node [thm, text width = 9.5em, below of = n25] (n15) {\textbf{1.5.} If
	$P_A$-avoiding, $\deg p > \deg q + 1$, not special,
	then strongly $P_A$-avoiding};

	\node [tool, text width = 8.2em, below of = n14] (n34) {\textbf{3.4.} Terms in $h^n$ where $h$ not special};
	\node [tool, text width = 8.2em, below of = n27] (n35) {\textbf{3.5} Orbit bounds if $\deg p > \deg q+1$};
	\path [arrow] (n21) -- (n25);
	\path [arrow] (n31) -- (n25);
	\path [arrow] (n33) -- (n27);
	\path [arrow] (n25) -- (n14);
	\path [arrow] (n25) -- (n27);
	\path [arrow] (n25) -- (n15);
	\path [arrow] (n34) -- (n15);
	\path [arrow] (n35) -- (n15);
\end{tikzpicture}
\end{center}

